The $\text{FP}^\text{NP}$ versus #P dichotomy for #EO

The complexity classification of the Holant problem has remained unresolved for the past fifteen years. Counting complex-weighted Eulerian orientation problems, denoted as #EO, is regarded as one of the most significant challenges to the comprehensive complexity classification of the Holant problem. This article presents an $\text{FP}^\text{NP}$ vs. #P dichotomy for #EO, demonstrating that #EO defined by a signature set is either #P-hard or polynomial-time computable with a specific NP oracle. This result provides a comprehensive complexity classification for #EO, and potentially leads to a dichotomy for the Holant problem. Furthermore, we derive three additional dichotomies related to the Holant problem from the dichotomy for #EO.

==> ppp.tex <==
\section{Acknowledgments}

The authors are grateful to  Shuai Shao and Zhuxiao Tang, for reading $f_{40}$ and $f_{56}$ to compare the progress of two groups, and at the same time, we keep the research independent. 
The authors would like to thank Pinyan Lu and Yaonan Jin, for discussing whether $\#\eo(f_{56})$ is in polynomial time together. 
The authors would like to thank Yicheng Pan, who pointed out the current counting argument in Lemma \ref{lem:alluphasdelta1}, which replaced the original long proof by induction method. 
All authors are supported by National Key R\&D Program of China (2023YFA1009500), NSFC 61932002 and NSFC 62272448. 



